Implementing Dynamic Answer Set Programming

We introduce an implementation of an extension of Answer Set Programming (ASP) with language constructs from dynamic (and temporal) logic that provides an expressive computational framework for modeling dynamic applications. Starting from logical foundations, provided by dynamic and temporal equilibrium logics over finite linear traces, we develop a translation of dynamic formulas into temporal logic programs. This provides us with a normal form result establishing the strong equivalence of formulas in different logics. Our translation relies on the introduction of auxiliary atoms to guarantee polynomial space complexity and to provide an embedding that is doomed to be impossible over the same language. Finally, the reduction of dynamic formulas to temporal logic programs allows us to extend ASP with both approaches in a uniform way and to implement both extensions via temporal ASP solvers such as telingo

==> Makefile <==
all: init
	latexmk paper.tex -pdf

watch: init
	latexmk paper.tex -pdf -pvc

clean:
	latexmk paper.tex -pdf -C

init: .initialized

SHELL=bash
.initialized:
	git config -f .gitmodules --get-regexp '^submodule\..*\.path$$' | \
	  while read path_key path_val; do \
	    url_key=$$(echo $$path_key | sed 's/\.path/.url/'); \
	    url=$$(git config -f .gitmodules --get "$$url_key"); \
	    git submodule add $$url $$path_val || true; \
	    git submodule update --init --recursive $$path_val; \
	  done
	touch .initialized

.PHONY: all watch clean init


==> tables/tab-translation.tex <==
\begin{table}
\centering\tiny
\begin{tabular}{|c|c|c|}\hline
  	$\mu$ &$\eta(\mu)$&$\pi(\mu)$ \\ \hline
		$\DDia{\top} \varphi$ & $\begin{array}{l}
					\alwaysF (\Lab{\mu} \leftrightarrow  \next \Lab{\varphi})\\
	  				\alwaysF \left(\finally   \to  \neg \Lab{\mu}\right)\\
				      \end{array}$ &  $\begin{array}{l}
							\wnext\alwaysF (\Lab{\mu}  \to \next \Lab{\varphi} )\\
	  						\wnext\alwaysF (\next \Lab{\varphi}  \to  \Lab{\mu} )\\
	  						\Lab{\mu}  \to \next \Lab{\varphi}\\
	  						\next \Lab{\varphi}  \to  \Lab{\mu}\\
	  						\alwaysF (\finally \to   \neg \Lab{\mu} )\end{array}$\\\hline

		$\DBox{\top}\varphi$ & $\alwaysF (\Lab{\mu} \leftrightarrow( \finally \vee \next \Lab{\varphi}))$ &
			$\begin{array}{l}
				\wnext \alwaysF (\Lab\mu \rightarrow \next \Lab{\psi} \vee \finally)\\
				\wnext \alwaysF (\next \Lab \psi \rightarrow \Lab\mu )\\
				\alwaysF (\finally \rightarrow \Lab\mu )\\
				\Lab\mu \rightarrow \next \Lab{\psi} \vee \finally\\
				\next \Lab \psi \rightarrow \Lab\mu \\
			\end{array}$\\\hline
%		$\DDia{\top^-} \varphi$ & $ \begin{array}{l}
%					\wnext\alwaysF (\Lab{\mu} \leftrightarrow \previous \Lab{\varphi})\\
%					\neg \Lab{\mu}
%					\end{array}$ & $\begin{array}{l}
%							\wnext\alwaysF (\Lab{\mu}  \to   \previous \Lab{\varphi} )\\
%							\wnext\alwaysF (\previous \Lab{\varphi}  \to  \Lab{\mu} )\\
%							\neg \Lab{\mu}
%							\end{array}$ \\\hline
%		$\DBox{\top^-}\varphi$ & $\alwaysF (\Lab{\mu} \leftrightarrow( \initially \vee \previous\Lab{\varphi}))$ & {\color{red}  $\begin{array}{ll}
%						\wnext\alwaysF (\Lab{\mu} \rightarrow \initially \vee \previous\Lab{\varphi})\\
%						\wnext\alwaysF (\Lab{\psi} \rightarrow \Lab{\mu})\\
%						\wnext\alwaysF (\initially \rightarrow \Lab{\mu})\\
%						\Lab{\mu} \rightarrow \initially \vee \previous\Lab{\varphi}\\
%						\initially \rightarrow \Lab{\mu}
%			\end{array}$}\\\hline
%%
		$\DDia{\varphi ? }\psi$ & $\alwaysF(\Lab{\mu} \leftrightarrow \Lab{\varphi} \wedge \Lab{\psi})$ & $\begin{array}{l}
											\wnext\alwaysF( \Lab{\mu}  \to   \Lab{\varphi} )\\
											\wnext\alwaysF( \Lab{\mu}  \to   \Lab{\psi} )\\
											\wnext\alwaysF( \Lab{\varphi} \wedge  \Lab{\psi}  \to   \Lab{\mu})\\
  											\Lab{\mu}    \to   \Lab{\varphi}\\
  											\Lab{\mu}   \to    \Lab{\psi} \\
  											\Lab{\varphi} \wedge \Lab{\psi}  \to  \Lab{\mu} \end{array}$\\\hline

	$ \DBox{\varphi?}\psi$ & $\alwaysF (\Lab{\mu} \leftrightarrow( \Lab{\varphi} \to \Lab{\psi}))$ & $\begin{array}{l}
									\wnext\alwaysF( \Lab{\mu}\wedge  \Lab{\varphi}  \to  \Lab{\psi})\\
 	    								\wnext\alwaysF(\neg \Lab{\varphi}  \to   \Lab{\mu} )\\
  	    								\wnext\alwaysF( \Lab{\psi}  \to   \Lab{\mu} )\\
  	    								\wnext\alwaysF(\top  \to   \Lab{\varphi}\vee\neg \Lab{\psi} \vee \Lab{\mu} ) \\
									\Lab{\mu}\wedge \Lab{\varphi}   \to   \Lab{\psi} \\
  	    								\neg \Lab{\varphi}  \to  \Lab{\mu}  \\
  	    								\Lab{\psi}    \to   \Lab{\mu}    \\
 	    								\Lab{\varphi}\vee \neg \Lab{\psi} \vee \Lab{\mu}\end{array}$ \\\hline

	$\DDia{\rho_1 + \rho_2} \varphi$ & $\alwaysF (\Lab{\mu} \leftrightarrow \DDia{\rho_1}\Lab{\varphi} \vee \DDia{\rho_2} \Lab{\varphi})$ & $\begin{array}{l}
	  							\wnext\alwaysF (\Lab{\mu}  \to  \DDia{\rho_1} \Lab{\varphi} \vee \DDia{\rho_2}  \Lab{\varphi})\\
	  							\wnext\alwaysF (\DDia{\rho_1}\Lab{\varphi}  \to  \Lab{\mu} )\\
	  							\wnext\alwaysF (\DDia{\rho_2}\Lab{\varphi}  \to  \Lab{\mu} )\\
	  							\Lab{\mu}  \to  \DDia{\rho_1} \Lab{\varphi} \vee \DDia{\rho_2}  \Lab{\varphi}\\
	  							\DDia{\rho_1}\Lab{\varphi}  \to  \Lab{\mu}\\
	  							\DDia{\rho_2}\Lab{\varphi}  \to  \Lab{\mu}
	  							\end{array}$\\\hline

	$\DBox{\rho_1 + \rho_2} \varphi$ & $\alwaysF (\Lab{\mu} \leftrightarrow \DBox{\rho_1}\Lab{\varphi} \wedge \DBox{\rho_2} \Lab{\varphi})$ & $\begin{array}{l}
									\wnext\alwaysF (\Lab{\mu}  \to  \DBox{\rho_1} \Lab{\varphi})\\
									\wnext\alwaysF (\Lab{\mu}  \to  \DBox{\rho_2}  \Lab{\varphi})\\
	  								\wnext\alwaysF (\DBox{\rho_1}\Lab{\varphi}  \wedge \DBox{\rho_2}\Lab{\varphi} \to  \Lab{\mu} )\\
									\Lab{\mu}  \to  \DBox{\rho_1} \Lab{\varphi}\\
									\Lab{\mu}  \to  \DBox{\rho_2}  \Lab{\varphi}\\
									\DBox{\rho_1}\Lab{\varphi}  \wedge \DBox{\rho_2}\Lab{\varphi} \to  \Lab{\mu}\\
	  								\end{array}$ \\\hline


	$\DDia{\rho_1;\rho_2} \varphi$ &  $\begin{array}{l}
\alwaysF (\Lab{\mu} \leftrightarrow \DDia{\rho_1}\Lab{\DDia{\rho_2}\varphi} )\\
\alwaysF (\Lab{\DDia{\rho_2}\varphi} \leftrightarrow \DDia{\rho_2}\Lab{\varphi})
	\end{array}$ & $\begin{array}{l}
					\wnext \alwaysF (\Lab{\mu} \rightarrow \DDia{\rho_1}\Lab{\DDia{\rho_2}\varphi} )\\
					\wnext \alwaysF (\DDia{\rho_1}\Lab{\DDia{\rho_2}\varphi} \rightarrow \Lab\mu )\\
					\wnext \alwaysF (\Lab{\DDia{\rho_2}\varphi} \rightarrow \DDia{\rho_2}\Lab{\varphi})\\
					\wnext \alwaysF (\DDia{\rho_2}\Lab{\varphi} \rightarrow \Lab{\DDia{\rho_2}\varphi})\\
					\Lab{\mu} \rightarrow \DDia{\rho_1}\Lab{\DDia{\rho_2}\varphi}\\
					\DDia{\rho_1}\Lab{\DDia{\rho_2}\varphi} \rightarrow \Lab\mu \\
					\Lab{\DDia{\rho_2}\varphi} \rightarrow \DDia{\rho_2}\Lab{\varphi}\\
					\DDia{\rho_2}\Lab{\varphi} \rightarrow \Lab{\DDia{\rho_2}\varphi}\\
					\end{array}$\\\hline
		$\DBox{\rho_1;\rho_2} \varphi$ & $\begin{array}{l}
										\alwaysF (\Lab{\mu} \leftrightarrow \DBox{\rho_1}\Lab{\DBox{\rho_2}\varphi} )\\
										\alwaysF (\Lab{\DBox{\rho_2}\varphi} \leftrightarrow \DBox{\rho_2}\Lab{\varphi} )
										\end{array}$
											& $\begin{array}{l}
												\wnext \alwaysF (\Lab{\mu} \rightarrow \DBox{\rho_1}\Lab{\DBox{\rho_2}\varphi} )\\
												\wnext \alwaysF (\DBox{\rho_1}\Lab{\DBox{\rho_2}\varphi} \rightarrow \Lab\mu )\\
												\wnext \alwaysF (\Lab{\DBox{\rho_2}\varphi} \rightarrow \DBox{\rho_2}\Lab{\varphi})\\
												\wnext \alwaysF (\DBox{\rho_2}\Lab{\varphi} \rightarrow \Lab{\DBox{\rho_2}\varphi})\\
												\Lab{\mu} \rightarrow \DBox{\rho_1}\Lab{\DBox{\rho_2}\varphi}\\
												\DBox{\rho_1}\Lab{\DBox{\rho_2}\varphi} \rightarrow \Lab\mu \\
												\Lab{\DBox{\rho_2}\varphi} \rightarrow \DBox{\rho_2}\Lab{\varphi}\\
												\DBox{\rho_2}\Lab{\varphi} \rightarrow \Lab{\DBox{\rho_2}\varphi}\\
												\end{array}$\\\hline
	$\DDia{\rho^*} \varphi$ & $\begin{array}{l}
				   \alwaysF( \Lab{\mu} \leftrightarrow \Lab{\varphi} \vee  \DDia{\rho} \Lab{\mu})\\
				   \alwaysF(\finally \to ( \Lab{\mu} \leftrightarrow \Lab{\varphi} ) )
				\end{array}$ & $\begin{array}{l}
								\wnext\alwaysF( \Lab{\mu} \to \Lab{\varphi} \vee \DDia{\rho}\Lab{\mu} )\\
  								\wnext\alwaysF (\DDia{\rho}\Lab{\mu} \to  \Lab{\mu})\\
        						\wnext\alwaysF(\Lab{\varphi}  \to  \Lab{\mu}  )\\
        						\Lab{\mu} \to \Lab{\varphi} \vee \DDia{\rho}\Lab{\mu}\\
        						\DDia{\rho} \Lab{\mu} \to  \Lab{\mu}\\
        						\Lab{\varphi}  \to  \Lab{\mu}\\
  								\alwaysF(\finally  \to (\Lab{\mu}\to\Lab{\psi} ) )\\
  								\alwaysF(\finally  \to ( \Lab{\psi}  \to  \Lab{\mu} ) )
								\end{array}$\\\hline
	$\DBox{\rho^*} \varphi$ & $\begin{array}{l}
				   \alwaysF( \Lab{\mu} \leftrightarrow \Lab{\varphi} \wedge  \DBox{\rho} \Lab{\mu})\\
				   \alwaysF(\finally \to ( \Lab{\mu} \leftrightarrow \Lab{\varphi} ) )
				\end{array}$ & $\begin{array}{l}
				\wnext\alwaysF( \Lab{\mu} \to \Lab{\varphi} )\\
				\wnext\alwaysF( \Lab{\mu} \to  \DBox{\rho}\Lab{\mu} )\\
				\wnext\alwaysF( \Lab{\varphi} \wedge \DBox{\rho} \Lab{\mu} \to  \DBox{\rho}\Lab{\mu} )\\
				\alwaysF(\finally  \to (\Lab{\mu}\to\Lab{\psi} ) )\\
				\alwaysF(\finally  \to ( \Lab{\psi}  \to  \Lab{\mu} ) )
				\end{array}$\\\hline
\end{tabular}
\caption{Normal form translation}
\label{tab:translation}
\end{table}
%
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

